Competency Questions and SPARQL-OWL Queries Dataset and Analysis

Competency Questions (CQs) are natural language questions outlining and constraining the scope of knowledge represented by an ontology. Despite that CQs are a part of several ontology engineering methodologies, we have observed that the actual publication of CQs for the available ontologies is very limited and even scarcer is the publication of their respective formalisations in terms of, e.g., SPARQL queries. This paper aims to contribute to addressing the engineering shortcomings of using CQs in ontology development, to facilitate wider use of CQs. In order to understand the relation between CQs and the queries over the ontology to test the CQs on an ontology, we gather, analyse, and publicly release a set of 234 CQs and their translations to SPARQL-OWL for several ontologies in different domains developed by different groups. We analysed the CQs in two principal ways. The first stage focused on a linguistic analysis of the natural language text itself, i.e., a lexico-syntactic analysis without any presuppositions of ontology elements, and a subsequent step of semantic analysis in order to find patterns. This increased diversity of CQ sources resulted in a 5-fold increase of hitherto published patterns, to 106 distinct CQ patterns, which have a limited subset of few patterns shared across the CQ sets from the different ontologies. Next, we analysed the relation between the found CQ patterns and the 46 SPARQL-OWL query signatures, which revealed that one CQ pattern may be realised by more than one SPARQL-OWL query signature, and vice versa. We hope that our work will contribute to establishing common practices, templates, automation, and user tools that will support CQ formulation, formalisation, execution, and general management.

==> heatmaps_analysis.tex <==

    
%\begin{figure}
%  \centering
%    \includegraphics[width=0.4\textwidth]{images/heatmap_0.png}
%  \caption{Similarity between patterns in different ontologies}
%  \label{fig:heatmap}
%\end{figure}

We also calculated the similarity between patterns defined for given ontologies, using Jaccard similarity over patterns with Equation~\ref{eq:jaccard}.


%The heatmap presented in Figure \ref{fig:heatmap} shows that there is a very low similarity between ontologies using that measure. The maximum similarity is obtained when comparing SWO with DMOP. The obtained Jaccard similarity is equal to: $0.058$.

\begin{equation}
    \texttt{JaccardSimilarity(A, B)} = \frac{1}{2}
  \label{eq:jaccard}
\end{equation}
where $\texttt{count\_shared(A, B)}$ counts occurences of patterns that are observed in both dataset A and dataset B, taking into consideration also multiple occurences of the same pattern and $\texttt{count\_total(A, B)}$ counts all occurences of patterns that are observed in dataset A and dataset B taking into consideration multiple occurences of the same pattern.

The maximum calculated similarity between patterns compared among different ontologies is very low, reaching it's maximum when comparing SWO and Dem@Care (0.259).



    %\item Aggregation level 3:  decide whether the question is open or yes/no type. If it is of the open type, is it the question about location, person, time, timespan, process, or general question? 

Heatmaps presented in Figures \ref{fig:heatmap1} and \ref{fig:heatmap2} present Jaccard's similarity of patterns in ontologies using different aggregation procedures 

\begin{figure}
  \centering
    \includegraphics[width=0.4\textwidth]{images/heatmap_lv1.png}
  \caption{Pattern similarity between different ontologies (Aggregation level 1)}
  \label{fig:heatmap1}
\end{figure}


\begin{figure}
  \centering
    \includegraphics[width=0.4\textwidth]{images/heatmap_lv2.png}
  \caption{Pattern similarity between different ontologies (Aggregation levels 1 + 2)}
  \label{fig:heatmap2}
\end{figure}


%\begin{figure}
%  \centering
%    \includegraphics[width=0.4\textwidth]{images/heatmap_lv1.png}
%  \caption{Pattern similarity between different ontologies (Aggregation level 3)}
%  \label{fig:heatmap3}
%\end{figure}



Table \ref{table:cq_similarity_levels} presents highest calculated Jaccard's similarity while comparing ontologies with different aggregations.

\begin{table}[h]
\begin{center}
\caption{Most similar ontologies on different level}
\label{table:cq_similarity_levels}.
 \begin{tabular}{ccc} 
 \hline
 Aggregation level & Most similar ontology pair & Score\\  
 \hline\hline
 No aggregation & SWO, Dem@Care & 0.259 \\
 \hline 
 1 & DMOP, Dem@Care & 0.441\\ 
 \hline
 1 + 2 & DMOP, Dem@Care & 0.5\\
 \hline
\end{tabular}
\end{center}
\end{table}

Although it is clear \AL{is it?} why grouping on level 1 is proposed, level 2 needs some further clarification.

We proposed Entity Chunks to be fragments of text that are likely to be represented in ontology. Sometimes it is not clear which fragment of text can state a single entity in ontology. Consider following CQ: \emph{Who owns the copyright for SIM?}.

In that case we cannot be sure what is the entity represented in the ontology: whether \textsf{copyright} and \textsf{SIM} are two separate entities? or \textsf{copyright for SIM} is a single entity? In general it is unclear how to interpret fragments in which two ECs are separated with a preposition - should they be separate ECs or should they be joined into one EC? In rules extracting ECs [TODO: REF] there is no preposition included, so by default when two entities are separated with it - our rules for EC always produce separate chunks.


%"Is Protege FOSS" can also be interpreted either as FOSS(Protege) or hasQuality(Protege, FOSS), 


%In previous sections we analyzed patterns defined as sequences of words with extracted chunks, but there is also alternative view on comparing CQs. Ren et. al. in the paper [REFERENCE] proposed a framework for patterns in which a set of features is extracted for every CQ to identify groups.

%Trying to apply the framework we realised, that on the level of pure CQs only Question Type, Question Polarity, Modifier and Domain Independent Element can be defined. The rest of features: Element Visibility, predicate arity and relation type depends on a given ontology, not the CQ itself. Different ontology modelling styles can lead to different feature values, so we had to omit those features. [ELABORATE MORE, WITH EXAMPLES]

%Working on a wider selection of CQs for more ontologies, we evaluated proposed framework for group identification among CQs.

==> others_comp.tex <==

\subsection{Grouping CQs in the context of framework proposed by Ren et al.}
An analysis of linguistic structures among patterns observed in the competency question dataset can also utilize the work of Ren et al. in order to verify if having collected more CQs we can observe some new categories of feature that are not previously identified due to limited dataset size.


 %%%% moved this part of analysis to related works
%.... Having collected more questions and ontologies than the paper of Ren et. al., we applied their framework in order to find groups of questions and verify whether some previously unobserved feature values manifest in our CQ dataset. ...
Trying to apply the features to our dataset we realised that on the level of CQ only four of them can be properly measured. For every competency question identification of values for features: Question Type, Question Polarity, Modifier, Domain Independent Element is easy, but capturing values of the rest of features is ontology-dependent, thus it is not possible to categorize the question properly without given existing ontology defined. 

Because that part of work focuses on analyzing CQs per se, without additional external contexts, we used only Question Type (QT), QuestionPolarity (QP), Modifier (MOD), Domain Independent Element(DINDE) to  group the collected CQ dataset and summarized it in Table~\ref{table:ren_framework}. 
%From the detected groups, the first one is shared among all ontologies, group 2 by all ontologies except Dem@Care and OntoDT, and groups  3, 5, 7, 10, 11, 12, 13, 14, 15, 16, 17 occur only in Software Ontology.

\begin{table*}[h]
\begin{center}
\caption{Patterns identified using features $1, 3, 6, 7$ from Ren's et. al. framework}
\label{table:ren_framework}.

 \begin{tabular}{cccccc} 
 \hline
 ID & Pattern example & QT & QP & MOD \\ %[0.5ex]
 \hline\hline
 1 & What EC does EC RC? & Selection & Positive & None  \\ % G1
 \hline
 2 & Does EC RC EC? & Binary & Positive & None \\ % G3
 \hline
 3 & Where is EC of EC? & Selection & Positive & None  \\ % G7
 \hline
 4 & How do I RC EC? & Selection & Positive & None  \\ % G2
 \hline
 5 & To what extent does EC RC EC? & Selection & Positive & None \\ % G13
 \hline
 7 & Who are EC of EC? & Selection & Positive & None  \\ % G 12
 \hline
 6 & Which EC RC exactly NUM EC? & Selection & Positive & Numeric \\ %G6
 \hline
 8 & What are the differences between EC of EC? & Selection & Positive & None  \\ % G5
 \hline
 9 & Are EC never EC? & Binary & Negative & None \\ % G4
 \hline
 10 & Is EC RC or not? & Binary & Both & None \\ % - G8
 \hline
 11 & How many EC do I RC to RC EC? & Count & Positive & None \\ % G14
 \hline
 12 & Which is the fastest EC RC EC? & Selection & Positive & Superlative  \\
 \hline
 13 & When was the NUM EC of EC RC? & Selection & Positive & Numeric \\
 \hline
 14 & How long has EC RC? & Selection & Positive & None  \\
 \hline
 15 & At what point did EC RC? & Selection & Positive & None  \\
 \hline
 16 & What EC is better for EC given EC as EC & Selection & Positive & Comparative \\
 \hline
 17 & What do others RC EC? & Selection & Positive & None \\
 \hline
 
\end{tabular}
\end{center}
\end{table*}

We have identified additional values that the measured features can have, they are listed below: \AL{I guess we could also add more question types, e.g. a \textbf{definition question}, asking about a definition. Another thing we could investigate to add is an entirely new category of, say, \textbf{Questions with signal words}, by analogy to \url{https://people.mpi-inf.mpg.de/~abujabal/publications/tempquestions/tempquestions.pdf}, page 19, but in our case, signal words would indicate the presence of logical operators like and, or, negation, quantifiers, which would indicate possible presence of particular SPARQL-OWL constructs in the query.}

\begin{itemize}
\item Domain Independent Element - the paper's authors mentioned two types of values: question about time and location. We propose to use also following values: person, period and procedure (although ontologies are not devoted to model procedures, there are some CQs in  multiple ontologies that ask about the way of performing given task).
\item Modifier - apart of asking about better/worser/best items, there are CQs that expect a list of differences as their output, so we propose an additional value: difference. Also there are some questions asking about an extent to which some task can be done, but that case is characteristic to Software Ontology only.
\end{itemize}

It is worth to mention that there are some cases in which we can categorize question's type as a binary, but from a pragmatic perspective instead of returning only yes/no value, some additional explanation should be provided. For instance, the answer "yes" for "Can I use some components of ppiStats for my software??" may be considered correct, but is uninformative, because most of people expects some list of components to be also returned from the ontology. The situation is different for questions like: "Does MATLAB work on 64 bit windows?" where simple yes/no answer is sufficient.


Altough we propose some extended categorization among remaining 4 features, after marking each question with the feature value, most of the questions fall into group one, constituing about 3/4 of our dataset.


==> preliminaries.tex <==
In this paper we consider ontologies represented in OWL 2 Web Ontology Language \cite{owl}.
We assume that the ontologies are consistent, i.e., there exists their respective models \cite{owl-direct-semantics}, and thus it is meaningful to query them.
An ontology can be serialized as an Resource Description Framework (RDF) graph \cite{owl-rdf-mapping} and thus queried using SPARQL Query Language  \cite{sparql}.
In its base form SPARQL is basically a pattern matching language and as such does not provide any reasoning capabilities, however, it is possible to introduce these by using SPARQL Entailment Regimes \cite{sparql-entailment-regimes}.
In particular, we employ OWL 2 Direct Semantics Entailment Regime.
Intuitively, it allows us to construct a SPARQL query such that its WHERE clause contains OWL axioms, possibly with some of its IRIs and literals replaced by SPARQL variables.
The results of the execution of such a query are all the variable mappings such that the axioms obtained by applying these mapping to the axioms in the query, are entailed by the queried ontology.

SPARQL, being a query language for RDF, employs Turtle syntax \cite{turtle} to express Basic Graph Patterns (BGPs) and this convention is kept also for expressing OWL axioms, i.e., their RDF representation is used \cite{owl-rdf-mapping}.
This is consistent with how the only available implementation behaves\footnote{\url{https://github.com/iliannakollia/owl-bgp}} \cite{DBLP:conf/esws/KolliaGH11,DBLP:journals/jair/KolliaG13}.

